Convergence properties of end invariants

We prove a continuity property for ending invariants of convergent sequences of Kleinian surface groups. We also analyze the bounded curve sets of such groups and show that their projections to non-annular subsurfaces lie a bounded Hausdorff distance from geodesics joining the projections of the ending invariants.

==> toplem.tex <==

\subsection{Topological lemmas}

In this section, we collect topological lemmas concerning ordering of curves and
surfaces in $S\times \R$ and derive applications which will be applicable to
split-level and pleated surfaces in our hyperbolic manifolds. 


\marginpar{More heuristic discussion needed eventually}

We begin by showing that a proper homotopy equivalence whose image is disjoint from a level curve
$\gamma_0=gamma\times \{ 0\}$ lies above $\gamma_0$ if and only if there is an essential curve on the surface which
intersects $\gamma$ whose image lies above $\gamma_0$.

\begin{lemma}{above and below}
Let $\alpha$ and $\gamma$ be overlapping curves on $S$ and let
$$f:(S, \boundary S) \to (S  \times \R, \boundary S \times \R)$$
be a homotopy equivalence with image disjoint from $\gamma_0=\gamma \times \{0\}$. Then $f(\alpha)$ lies above $\gamma_0$ if and only if $f$ lies above $\gamma_0$.
\end{lemma}

\begin{proof}
Clearly if $f$ lies above $\gamma_0$ then $f(\alpha)$ lies above $\gamma_0$. 

Suppose that $f(\alpha)$ lies above $\gamma_0$.
Let $A = \gamma \times (-\infty,0]$. We can homotope $f|_\alpha$,
in the complement of $\gamma_0$,
to a map whose image is disjoint from $A$. This homotopy can be extended to all of $S$ where the homotopy is supported on a neighborhood of $\alpha$ and the image of the homotopy is disjoint from $\gamma_0$. Let $g:(S,\boundary S) \to (S \times \R, \boundary S \times \R)$ be the new map. We can assume $g(S)$ intersects $A$ transversely. Then $\Gamma = g^{-1}(A)$ will be a collection of disjoint curves on $S$. Since $g$ is a homotopy equivalence every curve in $\Gamma$ will either be homotopic to 
$\gamma$ or will bound a disk. However, any curve that is homotopic to $\gamma$ must intersect $\alpha$ and since $g(\alpha)$ is disjoint from $A$ we must have that all curves in $\Gamma$ bound disks. Using the standard innermost disk argument and the fact that $(S \times \R) - \gamma_0$ is irreducible we can then homotope $g$, in the complement of $\gamma_0$, to a map whose image is disjoint from $A$. Such a map will lie above $\gamma_0$ so $g$ and therefore $f$ lies above $\gamma_0$.
\end{proof}

We next observe that a proper homotopy equivalence whose image is disjoint from an essential non-annular level
subsurface lies either above or below that subsurface

\begin{lemma}{above or below}
Let $W$ be a non-annular subsurface of a compact surface $S$.
If 
$$f:(S, \boundary S) \to (S  \times \R, \boundary S \times \R)$$
is a homotopy equivalence with image disjoint from $W_0=W \times \{0\}$,
then either $f(S)$ can be pushed to $+\infty $ or to $-\infty$ in the complement of
$W$.
\end{lemma}

\begin{proof}
Much as in the proof above, 
we may homotope $f$ (in the complement of $W_0$) so that its
intersection with each component of $\boundary W\times \R$ is a single simple closed curve.
Therefore, these intersections must all lie in $\boundary W\times (0,\infty)$ or all lie
in $\boundary W\times (-\infty,0)$. In the first case, $f(S)$ cannot intersect $W\times [0,\infty)$,
so on may  further push $f$ to $-\infty$ in the complement of $W_0$.
\end{proof}

It will also be useful to recall that an embedding of an essential subsurface with unknotted boundary
can be extended to a proper embedding of the entire surface which is isotopic to a level surface. This result
is a special case of Lemma 3.10 in \cite{ELC2}.
\marginpar{Mention Waldhausen?}

\begin{lemma}{unknotted subsurface}
Let $W$ be a compact essential subsurface of $S$. If \hbox{$h: W \to S \times \R$} is a $\pi_1$-injective embedding such that 
$h(\partial W)$ is unknotted, then $h$ extends to an embedding of $S$ in $S \times \R$ whose image 
is isotopic to $S \times \{0\}$.
\end{lemma}

\marginpar{This implies horizontal surfaces in product regions are correctly ordered. Say so?}


Our final topological lemma will be used to complete the proof of Theorem \ref{topistop} in the case
that the essential subsurface is an annulus.
\marginpar{Is there anything intuitive which can be said about the statement? Move to section 6?}

\begin{lemma}{both above}
Let $\gamma$ be a curve in $S$ and $\mathcal{N}(\gamma)$ be an open regular neighborhood of $\gamma \times \{1/2\}$ in 
$S \times [0,1]$ with boundary the torus $T$. Suppose that 
$$f:((S \times [0,1])\backslash \mathcal{N}(\gamma), T) \to ((S \times [0,1]) \backslash \mathcal{N}(\gamma), T)$$
is a continuous map such that 
\begin{enumerate}
\item
$f$ extends across $\mathcal{N}(\gamma)$,
\item 
$f$ restricted to $S \times \{0\}$ is homotopic to the inclusion map, in the complement of
$\mathcal{N}(\gamma)$,  and
\item 
the restriction of $f$ to both $S \times \{0\}$ and $S \times \{1\}$ lies above $\gamma \times \{1/2\}$.
\end{enumerate}
Then the restriction of $f$ to $T$ has degree zero.
\end{lemma}


\begin{proof}
Notice that we may assume that, after performing  a homotopy supported  in the complement of 
$\mathcal{N}(\gamma)$, that
$f(\boundary S \times [0,1]) \subseteq \boundary S \times [0,1]$ and that $f|_{S\times \{0\} }$ is the inclusion map.
Since $f(S\times \{1\})$ lies above $\gamma\times\{1/2\}$, we may homotope $f$,
again  by a homotopy with support in the complement of $\mathcal{N}(\gamma)$, so that  $f|_{S\times \{1\} }$
is a proper homotopy equivalence onto $S\times\{0\}$. Since $f|_{S\times\{0\} }$ is homotopic to the inclusion map and $f$ extends
across $\mathcal{N}(\gamma)$
we may further adjust $f$ so that $f(x,1)=(x,0)$ for all $x\in S$.
Thus, $f$ descends to a map
$$F: (S \times S^1)\backslash \mathcal{N}(\gamma) \to (S \times [0,1])\backslash \mathcal{N}(\gamma)$$
with $F(\boundary S \times S^1) \subseteq \boundary S \times [0,1]$.
Since $F$ defines a relative 3-chain in 
$$((S \times [0,1]) \backslash \mathcal{N}(\gamma), \boundary S \times [0,1]),$$
we see that
$$[F|_T]=0\in H_2((S \times [0,1])\backslash \mathcal{N}(\gamma), \boundary S \times [0,1]).$$
However, $[T]$ is a non-trivial homology class in 
\hbox{$H_2((S \times [0,1])\backslash \mathcal{N}(\gamma), \boundary S \times [0,1])$}
and 
$$F_*([T])=[F|_T]=d[T]$$
where $d$ is the degree of the restriction of $F$ to $T$ or, equivalently,
the degree of the restriction of $f$ to $T$. Therefore, this degree is zero.
\end{proof}




